Resilient Collaborative Privacy for Location-Based Services

Location-based Services (LBSs) provide valuable services, with convenient features for users. However, the information disclosed through each request harms user privacy. This is a concern particularly with honest-but-curious LBS servers, which could, by collecting requests, track users and infer additional sensitive user data. This is the motivation of both centralized and decentralized location privacy protection schemes for LBSs: anonymizing and obfuscating LBS queries to not disclose exact information, while still getting useful responses. Decentralized schemes overcome the disadvantages of centralized schemes, eliminating anonymizers and enhancing users' control over sensitive information. However, an insecure decentralized system could pose even more serious security threats than privacy leakage. We address exactly this problem, by proposing security enhancements for mobile data sharing systems. We protect user privacy while preserving accountability of user activities, leveraging pseudonymous authentication with mainstream cryptography. Our design leverages architectures proposed for large scale mobile systems, while it incurs minimal changes to LBS servers as it can be deployed in parallel to the LBS servers. This further motivates the adoption of our design, in order to cater to the needs of privacy-sensitive users. We provide an analysis of security and privacy concerns and countermeasures, as well as a performance evaluation of basic protocol operations showing the practicality of our design.

==> sections/adversary.tex <==
\section{System and Adversary Model}
\label{sec:adversary}




==> sections/conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we presented a decentralized secure and privacy protection scheme for \acp{LBS}. We leverage the concept of information sharing in \ac{P2P} systems for \ac{POI} information sharing, and further secure it in a privacy-preserving manner with pseudonym-based authentication. Through security and privacy analysis and performance evaluation, we show a system with high resiliency to different attacks and high practicality for the deployment. Our scheme can be extended in terms of optimizations we proposed. Each optimization needs to be designed more rigorously; and by doing simulation with the consideration of user mobility, we can quantify user privacy and determine optimal parameters for the optimizations. Incentive scheme and cross-checking mechanism can be integrated to promote user participation and improve attack resiliency.

==> sections/mobicrowd.tex <==
\section{MobiCrowd}
\label{sec:mobicrowd}

\subsection{Motivation}

There are many research studies on location privacy, which is an issue in many areas, such as \ac{LBS}, \ac{VC} and participatory sensing \cite{???}. For \ac{LBS}, many solutions rely on \textit{anonymizer}. An anonymizer is a \ac{TTP}, who has all the information regarding the queries, including historical and onging queries. Depending on an anonymizer, who has detailed information about the queries and more powerful computational capability, a better and more effective strategy can be designed to anonymize the queries; rather than depending on the clients, which has constrained resouce and limited information.

However, the problem is not solved by introducing an anonymizer. In other words, the anonymizer is introduced in order to prevent the \ac{LBS} server from misusing the information collected from the queries, but in fact, the problem is transfered from the \ac{LBS} server to the anonymizer. The anonymizer could still be the \textit{honest-but-curious} entity and do what the \ac{LBS} server could do.

==> sections/pseudo_auth.tex <==
\section{Our Scheme}
\label{sec:scheme}

The problems and requirements described in Sec. \ref{sec:problem} motivate the integration of \textit{pseudonym-based authentication} \cite{ps} into MobiCrowd. Though it was originally proposed for \ac{VC} domain, the idea is applicable to \acp{LBS} since it could compensate the imperfections of MobiCrowd. In the following, we explain how the pseudonymous authentication - both baseline scheme and \ac{GS}-based scheme, can be used in MobiCrowd to solve the problems and fulfill the requirments.

\subsection{\acf{BP} Scheme}
In \ac{BP} scheme, the \ac{CA}, who registered all the users, generates pseudonyms for them. The pseudonyms are signed by the \ac{CA} and the \ac{CA} maintains a table in which pseudonyms are mapped to the users whom the pseudonyms are issued to. However, if the \ac{CA} is an \textit{honest-but-curious} entity, it will be able to link the pseudonyms to the real identities of the owners. Therefore, being inspired by VeSPA \cite{vespa}, a Kerberized \ac{VPKI}, the roles of the \ac{CA} can be split into multiple \acp{CA}. In this way, a single \ac{CA} is not able to reveal the owners of the pseudonyms on its own.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figure/vespa_mobicrowd.pdf}
	\caption{MobiCrowd Leveraging Kerberized \ac{PKI}}
	\label{fig:vespa_mobicrowd}
\end{figure}


Each user is equipped with a long-term certificate, which is issued by the \ac{LTCA}, after being registered by the \ac{LTCA}. As shown in Fig. \ref{fig:vespa_mobicrowd}, a user can obtain pseudonyms through the steps 1-4. In other words, the user first obtains a ticket from the \ac{LTCA} and obtains pseudonyms with the ticket (see \cite{vespa} for more details).

In our scheme, a pseudonym, or a short-term credential, can be used to ensure the authenticity, protect the privacy and preserve the accountability of the user. The \ac{LBS} server and the neighbors who received the query can authenticate the user and the query with the pseudonym. With the pseudonym resolution protocol, the accountability of misbehaving users can be preserved.

%Next, we discuss the utilization of \ac{GS} scheme and \ac{HP} scheme - the combination of \ac{BP} and \ac{GS} schemes.

\subsection{\acf{GS} scheme}

In the \ac{GS} scheme, each user is equipped with a group signing key \textit{gsk}, which is used to sign messages. The signatures generated with any $gsk$ in the group , can be verified with group public key \textit{gpk}, which is unique in the group. Moreover, the signatures generated with same $gsk_i$ cannot be linked. The \ac{GM}, who generated all the keys, can reveal the identity of the signer if needed. With the \ac{GS} scheme, a user could authenticate itself pseudonymously to the \ac{LBS} server and her neighbors. A query is signed by the user with $gsk_i$ and sent to the \ac{LBS} server or her neighbors. Upon receipt of the query, the nodes who received the query could verify the query with $gpk$, and they do not know who is the signer. They only know the signer is a legitimate user in the system, and they will reply accordingly. The accountability of users could be achieved with the help of \ac{GM}.

In \cite{Manolopoulos:2013:STI:2436196.2436213}, the \ac{GS} scheme is deployed in cellular network in order to protect user privacy. Compared to the difficulty of introducing and deploying new infrastructures for the \ac{BP} scheme; the \ac{GS} scheme relies on existing cellular infrastructures, which could shorten the deployment phase.

A drawback of the \ac{GS} scheme is that the cryptographic operations are not efficient \cite{ps}. However, for \acp{LBS}, where requirement for real-time response is not a main factor, the processing delays in the \ac{GS} scheme are acceptable.

\subsection{\acf{HP} Scheme}

In the \ac{HP} scheme, pseudonyms are generated \textit{on-the-fly} leveraging the \ac{GS} scheme. A user generates public/private key pairs and sign the public keys with her $gsk_i$. Then, the signed public keys are used as \textit{pseudonymous certificates}. A node in the group, who received a message attached with a pseudonymous certificate, could verify the pseudonymous certificfate with the \textit{gpk} and then verify the message with the public key in the pseudonymous certificate.

In \cite{ps}, the \ac{HP} scheme is proposed in order to reduce the overhead and fit the requirements of safety applications in \ac{VC} domain. However, as described earlier, the processing delays of the \ac{GS} scheme are acceptable in \acp{LBS}, and using the \ac{HP} scheme will introduce extra overhead by verifying the pseudonymous certificate. Moreover, three optimizations, proposed in \cite{ps} for reducing the overhead of the \ac{HP} scheme in high-frequency beacon transmissions, are not applicable to \acp{LBS}.

However, as mentioned in Sec. \ref{sec:introduction}, it is possible that \acp{LBS} will be integrated into \acp{ITS}, and passengers who have smartphones will be involved in the \acp{ITS}. In this case, the nodes in MobiCrowd are not limited to smartphones; vehicles, or more specifically, \acp{OBU} can be considered as ndoes in MobiCrowd as well. Therefore, for the vehicles, they can use the same pseudonyms they are using for signing beacons. By using the \ac{HP} scheme and the optimizations, for P2P queries between vehicles, a vehicle who received a qeury could have already cached the pseudonym, under which the received query is signed. Therefore, the vehicle could verify the query immediately without verifying the pseudonym. For the queries sent from the smartphones, they could still be signed under \ac{GS} scheme, since the optimizations are not applicable. In other words, for the queries sent from vehicles, they can be signed with pseudonyms, while the queries from the smartphones are signed with group signing keys.

==> sections/related.tex <==
\section{Problem Statement and Related Work}
\label{sec:problem}


